Interpretable Causal Inference for Analyzing Wearable, Sensor, and Distributional Data

Many modern causal questions ask how treatments affect complex outcomes that are measured using wearable devices and sensors. Current analysis approaches require summarizing these data into scalar statistics (e.g., the mean), but these summaries can be misleading. For example, disparate distributions can have the same means, variances, and other statistics. Researchers can overcome the loss of information by instead representing the data as distributions. We develop an interpretable method for distributional data analysis that ensures trustworthy and robust decision-making: Analyzing Distributional Data via Matching After Learning to Stretch (ADD MALTS). We (i) provide analytical guarantees of the correctness of our estimation strategy, (ii) demonstrate via simulation that ADD MALTS outperforms other distributional data analysis methods at estimating treatment effects, and (iii) illustrate ADD MALTS' ability to verify whether there is enough cohesion between treatment and control units within subpopulations to trustworthily estimate treatment effects. We demonstrate ADD MALTS' utility by studying the effectiveness of continuous glucose monitors in mitigating diabetes risks.

==> cate.tex <==
\begin{align*}
    &\text{for } i = 1, \ldots, 1000: \\
                  &\hspace{2mm} x_{i,1}, \ldots, x_{i,10} \sim Unif[-1,1] \\
                  &\hspace{2mm} F_{x_{i, 1}}, \ldots, F_{x_{i,10}} = \delta_{x_{i,1}}, \ldots, \delta_{x_{i,10}} \\
                  &\hspace{2mm} t_i \sim \text{Bern}\left( \text{expit}\left( x_{i,1} + x_{i,2} \right) \right), \varepsilon_Y \sim \mathcal{N}(0,1) \\
                  &\hspace{2mm} \alpha(t_i) = 5 + 10\sin(\pi x_{i,1} + x_{i,2})^2 + 20(x_{i,3} - 0.5)^2 \\
                  &\hspace{2mm} + 10x_{i,4} + 5x_{i,5} + t_i10x_{i,3}\cos(\pi x_{i,1} x_{i,2})^2+ \varepsilon_Y \\
                  &\hspace{2mm} \text{for } j = 1, \ldots, 1001: \\
                  &\hspace{2mm} \hspace{2mm} z_{i,j} \sim \text{Bern}(1/4) \\
                  &\hspace{2mm} \hspace{2mm} y_{i,j}(0) \sim \text{Beta}( 2\alpha(0), 8\alpha(0) )^{z_{i,j}}\text{Beta}( 8\alpha(0), 2\alpha(t_i))^{1-z_{i,j}} \\
                  &\hspace{2mm} \hspace{2mm} y_{i,j}(1) \sim \text{Beta}( 2\alpha(1), 8\alpha(1) )^{1-z_{i,j}}\text{Beta}( 8\alpha(1), 2\alpha(1))^{z_{i,j}} \\
                  &\hspace{4mm} F_{Y_i}^{-1}(q) = \min \{y : \frac{1}{1001}\sum_{j = 1}^{1001} \mathbf{1}[y_{i,j}(t_i) \leq y] \geq q \}.
\end{align*}

The DGP has 10 scalar covariates that are transformed to degenerate distributions. We then assign treatment using a simple, linear propensity score model using two of the covariates. Our outcome is a mixture of two Beta distributions whose parameters are controlled by the term $\alpha(t_i)$; $\alpha(t_i)$ is a combination of complex quadratic and trignometric terms. When $t_i = 1,$ the mixture proportions flip so that more mass is concentrated in the upper end of the distribution's support; additionally, when $t_i = 1$, the Beta distribution's parameter increases by another complex interaction of trignometric terms, causing the variance of each mixture component shrink. We construct each unit's observed quantile function using the outcome observations associated with unit $i$'s treatment status: $y_{i,1}(t_i), \ldots, y_{i,1001}(t_i)$. In our DGP, we have 5 relevant covariates and 5 irrelevant covariates. Figure \ref{fig:potentialOutcomes} displays an example of the treated and control potential outcome distributions for a single unit in this DGP.



\begin{figure}
    \centering
    \includegraphics[width=0.45\textwidth]{plots/potential_outcomes.png}
    \caption{Example of the treated (orange) and control (blue) potential outcome distributions under the data generating process. The treatment causes the mixture proportion to change and affects the parameter of the Beta distribution. As $\alpha(t_i)$ increases, the variance of each mixture decreases.}
    \label{fig:potentialOutcomes}
\end{figure}



We evaluate ADD MALTS' CATE estimation ability to a series of baselines. As proposed in \cite{lin2021causal}, we perform outcome regression using linear regression for each quantile of the outcome function (LR). We also fit two different propensity score models: a linear propensity score model (Lin PS) and a non-paremetric propensity score using a random forest (RF PS). We combine the outcome regression with the parametric and non-parametric propensity scores using \cite{lin2023causal}'s doubly robust formulation (LR + Lin PS, LR + RF PS). We also perform propensity score matching with the linear propensity score model (Lin PSM). Lastly, we fit outcome regression models using \cite{qiu2022random}'s Fr\'echet tree (FT) and Fr\'echet random forest (FRF) algorithms for functional outcomes. We measure estimation performance using a generalization of the relative error metric for functional data, the Integrated Relative Error (IRE). 
\begin{align*}
IRE(\%) = 100 \cdot \int_0^1 \frac{(\hat{\tau}(q|F_{\bm{x}_i}) - \tau(q|F_{\bm{x}_i}))^2}{\tau(q|F_{\bm{x}_i})^2}dq.
\end{align*}
We repeated our experiment over 100 monte carlo iterations; in each iteration, 20\% of the data was used to train each algorithm while 80\% was used to estimate treatment effects.

\begin{figure}
    \centering
    \includegraphics[width=0.47\textwidth]{plots/cate_estimation.png}
    \caption{Integrated relative error (IRE) for each estimation strategy across 100 monte carlo simulations. ADD MALTS outperforms all other methods.}
    \label{fig:cate_estimation}
\end{figure}

Figure \ref{fig:cate_estimation} displays the IRE for each estimation strategy. \textbf{ADD MALTS outperforms all other methods}, with a median IRE of just 13.15\%. In comparison, the highly flexible and non-parametric tree-based methods (FT and FRF) require sacrifices in estimation performance, achieving a median IRE of about 46\%. Furthermore, ADD MALTS does significantly better than linear propensity score matching and the doubly robust methods, even when the true propensity score model is also linear. By construction of the IRE metric, these results suggest that ADD MALTS is able to estimate the treatment effect at \textit{all} quantiles incredibly well, even at the tails of the distribution.


==> checklist.tex <==
\section*{Checklist}

 \begin{enumerate}


 \item For all models and algorithms presented, check if you include:
 \begin{enumerate}
   \item A clear description of the mathematical setting, assumptions, algorithm, and/or model. [\framebox{Yes}/No/Not Applicable]. Section~\ref{sec:background} discuss the mathematical settings and some assumptions. Section~\ref{sec:framework} discusses our other assumptions and methodology.
   \item An analysis of the properties and complexity (time, space, sample size) of any algorithm. [Yes/\framebox{No}/Not Applicable] Section \ref{sec:timing} in the appendix shows runtimes for our algorithm across different simulation setups.
   \item (Optional) Anonymized source code, with specification of all dependencies, including external libraries. [\framebox{Yes}/No/Not Applicable]. All code can be found here: \href{https://github.com/almost-matching-exactly/addmalts}{https://github.com/almost-matching-exactly/addmalts}.
 \end{enumerate}


 \item For any theoretical claim, check if you include:
 \begin{enumerate}
   \item Statements of the full set of assumptions of all theoretical results. [\framebox{Yes}/No/Not Applicable]. Sections~\ref{sec:background} state the full assumptions necessary for Proposition~\ref{prop:identification}. Section ~\ref{sec:framework} state the relevant assumptions for Lemma~\ref{lemma:barycenter_consistency} and Theorem~\ref{thm:cate_consistency}.
   \item Complete proofs of all theoretical results. [\framebox{Yes}/No/Not Applicable]. Appendix~\ref{sec:identificationATE} and ~\ref{sec:CATEconsistency} provide the proofs of our theoretical claims.
   \item Clear explanations of any assumptions. [\framebox{Yes}/No/Not Applicable]. Section~\ref{sec:background} explains the assumptions needed to identify average treatment effects (Proposition~\ref{prop:identification}). Section~\ref{sec:framework} discusses Assumption~\ref{assm:smoothness} needed to consistently estimate conditional average treatment effects using ADD MALTS.
 \end{enumerate}


 \item For all figures and tables that present empirical results, check if you include:
 \begin{enumerate}
   \item The code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL). [\framebox{Yes}/No/Not Applicable]. All code can be found here: \href{https://github.com/almost-matching-exactly/addmalts}{https://github.com/almost-matching-exactly/addmalts}.
   \item All the training details (e.g., data splits, hyperparameters, how they were chosen). [\framebox{Yes}/No/Not Applicable] Appendix sections~\ref{sec:cate_exp_details} and \ref{sec:positivity_exp_details} provide more details. Code also includes comments.
    \item A clear definition of the specific measure or statistics and error bars (e.g., with respect to the random seed after running experiments multiple times). [\framebox{Yes}/No/Not Applicable]
    Contents of each plot is described in the corresponding caption.
    \item A description of the computing infrastructure used. (e.g., type of GPUs, internal cluster, or cloud provider). [\framebox{Yes}/No/Not Applicable]
    Appendix Sections~\ref{sec:comp_resources} provide more details.
 \end{enumerate}

 \item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets, check if you include:
 \begin{enumerate}
   \item Citations of the creator If your work uses existing assets. [\framebox{Yes}/No/Not Applicable] 
   \item The license information of the assets, if applicable. [Yes/No/\framebox{Not Applicable}]
   \item New assets either in the supplemental material or as a URL, if applicable. [Yes/No/\framebox{Not Applicable}]
   \item Information about consent from data providers/curators. [\framebox{Yes}/No/Not Applicable]
   \item Discussion of sensible content if applicable, e.g., personally identifiable information or offensive content. [Yes/No/\framebox{Not Applicable}]
 \end{enumerate}

 \item If you used crowdsourcing or conducted research with human subjects, check if you include:
 \begin{enumerate}
   \item The full text of instructions given to participants and screenshots. [Yes/No/\framebox{Not Applicable}]
   \item Descriptions of potential participant risks, with links to Institutional Review Board (IRB) approvals if applicable. [Yes/No/\framebox{Not Applicable}]
   \item The estimated hourly wage paid to participants and the total amount spent on participant compensation. [Yes/No/\framebox{Not Applicable}]
 \end{enumerate}

 \end{enumerate}

==> dist_cov_experiment.tex <==
\begin{table*}[t] \label{tbl:dgps}
    \centering
    \begin{tabular}{c|c|c}
        \textbf{Name} & $\mathbf{\mu}$ & $\mathbf{\sigma}$  \\
        \hline
        Variance & $10 + x_{i,0} + 2x_{i,1} + \varepsilon_i$ & $\left|10 + x_{i,0} + 2x_{i,1} + 10T_i + \varepsilon_i \right|$ \\
        \hline
        Linear & $10 + x_{i,0} + 2x_{i,1} + 10T_i + \varepsilon_i$ & 1 \\
        \hline
        Complex & $\begin{matrix}
        10\sin\left(\pi x_{i,0}x_{i,1} \right) + 20(x_{i,2} - 0.5)^2 + 10x_{i,3} + 5x_{i,4} \\
        + T_i\left\{7 + x_{i,2}\cos\left(\pi x_{i,0}x_{i,1}\right) \right\} + \varepsilon_i
                    \end{matrix} $ & $\left|10 + x_{i,0} + 2x_{i,1} + \varepsilon_i\right|$ \\
        \hline
        Dist Cov & $\begin{matrix}
        10\sin\left(\pi \left[\int_0^1F_{x_{i,0}}^{-1}(q) dq \right]x_{i,1} \right) + 20(x_{i,2} - 0.5)^2 + 10x_{i,3} + 5x_{i,4} \\
        + T_i\left\{7 + x_{i,2}\cos\left(\pi \left[\int_0^1F_{x_{i,0}}^{-1}(q) dq \right]x_{i,1}\right) \right\} + \varepsilon_i
                    \end{matrix} $ & 1
    \end{tabular}
    \caption{In our simulations, the distributional outcomes are truncated normal distributions (truncated at $\pm 3$ standard deviations from the mean). The table describes the functions used to generate the mean and variance of each outcome. The first three simulations have 10 scalar covariates $x_{i,0}, \ldots, x_{i,9}.$ The last simulation (Dist Cov) has a distributional covariate $F_{x_{i,0}}$, which we use by taking the integral of its cumulative distribution function as a covariate, and 9 scalar covariates $x_{i,1}, \ldots, x_{i,9}.$}
    \label{tab:my_label}
\end{table*}

\begin{figure*}[t] \label{fig:cate_estimation_collated}
    \centering
    \includegraphics[width=0.8\textwidth]{plots/collated_cate_estimation_mire.png}
    \caption{The figure displays the Integrated Relative Error (\%) of the different methods we consider for the simulation setups detailed in Table \ref{tbl:dgps}.}
\end{figure*}

We consider four data generative processes (DGPs). In each DGP, we generate our distributional outcomes as truncated normal distributions (truncated at $\pm 3$ standard deviations from the mean). Table \ref{tbl:dgps} describes the functions used to generate the means and variances of the truncated normal outcomes for each DGP. In the ``Linear,'' ``Variance,'' and ``Complex'' DGPs, we sample 10 \textit{scalar} covariates $x_{i,0}, \ldots, x_{i,9}$, independently and identically from \textit{Uniform}$[-1,1].$ The propensity score models are linear: $\mathbb{P}(T_i = 1 | F_{\bm{x}_i}) = \text{expit}(x_{i,0} + x_{i,1}).$

The ``Dist Cov'' simulation instead has nine scalar covariates and a distributional covariate $F_{x_{i,0}}$. $F_{x_{i,0}}$ is uniformly sampled to be any uniform distribution between $[-1,0]$ and $[-1,1].$ We use the integral of the quantile function as a feature to generate outcomes. Because baseline methods can only handle scalar covariates, we instead provide them the preprocessed covariate, the area under the quantile function. Here, the propensity score model is also linear but depends on this processed distribution: $\mathbb{P}(T_i = 1|F_{\bm{x}_i}) = $


For each DGP, we consider 1500 units, using $67\%$ in the training set and $33\%$ to estimate CATEs. Also, each DGP has at least five irrelevant covariates. We repeat each experiment 100 times and evaluate CATE estimation performance using the $\text{Integrated Relative Error (\%)} = 100 \cdot \int_0^1 \left| \frac{\hat{\tau}(q) - \tau(q)}{\tau(q)} \right|dq$.

We compare ADD MALTS to the following baselines: \textbf{Lin PSM} and \textbf{RF PSM} represent propensity score matching fit with linear and random forest models, respectively; \textbf{FT} and \textbf{FRF} represent decision tree and random forest methods for functional outcomes \citep{qiu2022random}; \textbf{LR} represents outcome regression fit at each quantile with a linear regression \citep{lin2023causal}; \textbf{LR + Lin PS} and \textbf{LR + RF PS} represent augmented inverse propensity weighting methods combining the linear outcome regression with linear and random forest propensity score models, respectively.

Figure \ref{fig:cate_estimation_collated} displays the results of our simulations. The y-axis represents the integrated relative error so lower means better performance. Across the board, ADD MALTS performs at least as well as the baselines. \textbf{In the more complex simulations, ADD MALTS completely outperforms competing methods.} For the ``Complex'' simulation, ADD MALTS achieves a median IRE of only 41.7\%, \textbf{reducing the error from the next best method by one-third} (LR + RF PSM, LR + Lin PSM with median of $\approx 115\%$).

In the ``Dist Cov`` DGP, the mean of the outcome is calculated using the processed distribution. In practice, the correct way to process the distribution is unknown, but we advantage the baseline methods by letting them use this unrealistic information. ADD MALTS only has access to the raw distribution. Even in this scenario, ADD MALTS outperforms the baselines.
ADD MALTS' achieves a median IRE of only 47\%, demonstrating that \textbf{ADD MALTS can effectively handle both scalar and distributional covariates}. ADD MALTS does not require us to process or summarize distributions; instead, we only need to calculate distances between them. ADD MALTS handles the complex data without sacrificing performance.

Because IRE describes the error across the entire function, our simulation/evaluation also highlights ADD MALTS' ability to estimate CATEs accurately at tails also. ADD MALTS achieves higher performance than competing methods because it is not susceptible to model misspecification and overfitting.



